DGInStyle: Domain-Generalizable Semantic Segmentation with Image Diffusion Models and Stylized Semantic Control

Large, pretrained latent diffusion models (LDMs) have demonstrated an extraordinary ability to generate creative content, specialize to user data through few-shot fine-tuning, and condition their output on other modalities, such as semantic maps. However, are they usable as large-scale data generators, e.g., to improve tasks in the perception stack, like semantic segmentation? We investigate this question in the context of autonomous driving, and answer it with a resounding "yes". We propose an efficient data generation pipeline termed DGInStyle. First, we examine the problem of specializing a pretrained LDM to semantically-controlled generation within a narrow domain. Second, we propose a Style Swap technique to endow the rich generative prior with the learned semantic control. Third, we design a Multi-resolution Latent Fusion technique to overcome the bias of LDMs towards dominant objects. Using DGInStyle, we generate a diverse dataset of street scenes, train a domain-agnostic semantic segmentation model on it, and evaluate the model on multiple popular autonomous driving datasets. Our approach consistently increases the performance of several domain generalization methods compared to the previous state-of-the-art methods. The source code and the generated dataset are available at https://dginstyle.github.io.

==> figs/controlnet_style_overfit.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth,trim={0 0 0 0},clip]{img/style_overfit.pdf}
    \caption{
    \textbf{
    ControlNet learns the source domain style.
    }
    This effect hinders varied data generation for domain generalization. 
    The proposed Style Swap preserves the diversity of the prior domain. }
    \label{fig:controlnet-style}
\end{figure}

==> figs/styles.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth,trim={0 0 0 0},clip]{img/styles_v2.jpg}
    \caption{
    \textbf{Style variations.}
    DGInStyle can generate various scene conditions using style prompting. 
    The same condition mask is used to illustrate the pixel-perfect alignment of the generations.
    }
    \label{fig:styles}
\end{figure}

==> tab/ablation.tex <==
\begin{table}[t!]
\centering
\renewcommand{\arraystretch}{1.3}
\setlength{\tabcolsep}{15pt}
\resizebox{\columnwidth}{!}{
\begin{tabular}{cccc c cc}
\toprule
\multicolumn{4}{c}{Modules} && \multicolumn{2}{c}{mIoU$\uparrow$} \\
MRLF    & Style Swap   &  Style Prompts & RCG   && Avg3 & Avg5 \\ \hline
\ding{56}& \ding{56}&\ding{56}&\ding{56}&& 51.46 & 43.31 \\
\ding{52}& \ding{56}&\ding{56}&\ding{56}&& 52.84 & 44.27 \\
\ding{52}& \ding{52}&\ding{56}&\ding{56}&& 53.85 & 45.84 \\
\ding{52}& \ding{52}&\ding{52}&\ding{56}&& 53.95 & 46.16 \\ 
\ding{52}& \ding{52}&\ding{52}&\ding{52}&& \textbf{54.25} & \textbf{46.47}\\ 

\midrule

\mycrossmark & \mycheckmark & \mycheckmark & \mycheckmark && 53.07 & 45.19 \\
\mycheckmark & \mycrossmark & \mycheckmark & \mycheckmark && 51.50 & 43.12 \\
\mycheckmark & \mycheckmark & \mycrossmark & \mycheckmark && 53.85 & 44.67 \\
\mycheckmark & \mycheckmark & \mycheckmark & \mycrossmark && 53.95 & 46.16 \\
\mycheckmark & \mycheckmark & \mycheckmark & \mycheckmark && \textbf{54.25} & \textbf{46.47} \\

\bottomrule
\end{tabular}
}
\caption{
\textbf{Ablation studies} on different components for our data generation pipeline. All models use DAFormer~\cite{hoyer2022daformer} and are trained with GTA and our generated dataset. MRLF: our multi-resolution latent fusion module; RCG: using rare class sampling in the ControlNet training and dataset generation phases.}
\label{tab:ablation}

\end{table}
